ZeRO++: Extremely Efficient Collective Communication for Giant Model Training

Zero Redundancy Optimizer (ZeRO) has been used to train a wide range of large language models on massive GPUs clusters due to its ease of use, efficiency, and good scalability. However, when training on low-bandwidth clusters, or at scale which forces batch size per GPU to be small, ZeRO's effective throughput is limited because of high communication volume from gathering weights in forward pass, backward pass, and averaging gradients. This paper introduces three communication volume reduction techniques, which we collectively refer to as ZeRO++, targeting each of the communication collectives in ZeRO. First is block-quantization based all-gather. Second is data remapping that trades-off communication for more memory. Third is a novel all-to-all based quantized gradient averaging paradigm as replacement of reduce-scatter collective, which preserves accuracy despite communicating low precision data. Collectively, ZeRO++ reduces communication volume of ZeRO by 4x, enabling up to 2.16x better throughput at 384 GPU scale.

==> text/comm_analysis.tex <==
% \section{ZeRO++ Communication Volume Analysi}

% \textcolor{blue}{Guanhua: I also don't know why we need a whole section for communication volume analysis, which is simple. As we discussed and agreed, this should be last subsection of design}
% \subsection{DP and ZeRO Communication Volume}
% \subsection{ZeRO++ Commnunication Volume}
% \subsubsection{hpz}
% \subsubsection{quantized weights}
% \subsubsection{quantized gradients}

==> text/discuss.tex <==
\section{Discussion and limitation}

\begin{itemize}
    \item this work is not limited to zero stage 3. We can regard it as low-latency replacement for collectives such as all-gather and reduce-scatter. 
    \item The only case where there will be little gain is small model with large batch size on cutting-edge cluster, which is rare
    \item model convergence impact, future work: more advance and efficient quant algorithm. 
\end{itemize}
